Fine-grain atlases of functional modes for fMRI analysis

Population imaging markedly increased the size of functional-imaging datasets, shedding new light on the neural basis of inter-individual differences. Analyzing these large data entails new scalability challenges, computational and statistical. For this reason, brain images are typically summarized in a few signals, for instance reducing voxel-level measures with brain atlases or functional modes. A good choice of the corresponding brain networks is important, as most data analyses start from these reduced signals. We contribute finely-resolved atlases of functional modes, comprising from 64 to 1024 networks. These dictionaries of functional modes (DiFuMo) are trained on millions of fMRI functional brain volumes of total size 2.4TB, spanned over 27 studies and many research groups. We demonstrate the benefits of extracting reduced signals on our fine-grain atlases for many classic functional data analysis pipelines: stimuli decoding from 12,334 brain responses, standard GLM analysis of fMRI across sessions and individuals, extraction of resting-state functional-connectomes biomarkers for 2,500 individuals, data compression and meta-analysis over more than 15,000 statistical maps. In each of these analysis scenarii, we compare the performance of our functional atlases with that of other popular references, and to a simple voxel-level analysis. Results highlight the importance of using high-dimensional "soft" functional atlases, to represent and analyse brain activity while capturing its functional gradients. Analyses on high-dimensional modes achieve similar statistical performance as at the voxel level, but with much reduced computational cost and higher interpretability. In addition to making them available, we provide meaningful names for these modes, based on their anatomical location. It will facilitate reporting of results.

==> Makefile <==
LATEX=pdflatex -synctex=1
LATEXOPT=--shell-escape
NONSTOP=--interaction=nonstopmode

LATEXMK=latexmk
LATEXMKOPT=-pdf -view=none
CONTINUOUS=-pvc

MAIN=paper

FIGURES := $(shell find figures -type f)
BIB=biblio.bib

SOURCES=$(MAIN).tex $(FIGURES) $(BIB)

$(MAIN).pdf $(MAIN).bcf: $(MAIN).tex $(SOURCES) figures figures/abstract.pdf
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

figures/abstract.pdf:
	inkscape --file=drawings/abstract.svg --export-area-drawing --without-gui --export-pdf=figures/abstract.pdf

$(MAIN)_embed.pdf: $(MAIN).pdf
	gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite \
	-sOutputFile=$(MAIN)_embed.pdf $(MAIN).pdf
	
clean:
	$(LATEXMK) -C $(MAIN)
	rm -f $(MAIN).pdfsync
	rm -rf *~ *.tmp
	rm -f *.bbl *.blg *.aux *.end *.fls *.log *.out \
	*.fdb_latexmk *.synctex.gz *.synctex.gz\(busy\) *.lol *.xml
	rm -f $(MAIN)-blx.bib
	rm -f $(MAIN)_embed.pdf
	rm -rf hal hal.zip
	rm *.spl
extracted.bib: $(MAIN).pdf
	biber -g tools/biber.conf --output-format=bibtex $(MAIN).bcf -O $@

hal.zip:
	bash tools/make_hal.sh

$(MAIN)_main.pdf $(MAIN)_supp.pdf: $(MAIN)_embed.pdf
	pdftk $(MAIN)_embed.pdf cat 1-10 output $(MAIN)_main.pdf
	pdftk $(MAIN)_embed.pdf cat 11-end output $(MAIN)_supp.pdf

watch: $(MAIN).tex $(SOURCES)
	$(LATEXMK) $(LATEXMKOPT) -pdflatex="$(LATEX) $(LATEXOPT) %O %S" $(MAIN)

count: 
	texcount $(MAIN).tex

.PHONY: all clean watch count



==> validation.tex <==
%!TEX root = paper.tex
\section{Experimental study: validating the multi-scale atlases}

\arthur{Kamalakar, can you put every paragraph of 4. into their counterpart in 3., in a paragraph "Data.", skipping all details and putting them into the appendix ? I think it would be much more readable}

\subsection{Validation datasets}
We apply our data analysis pipelines on large and publicly available fMRI
datasets which includes task-fMRI \citep{chang2015emotion} and rs-fMRI
\citep{mueller2005, vanessen2012hcpdata, craddockneurobureau, calhoun2012}.
We detail below about these datasets according to each pipeline.

\begin{table}[t]
    \small
    \begin{center}
        \begin{tabular}{c|c|c}
            \hspace*{0.3em}\cellcolor{gray!25}\bf{Task-fMRI} &
            \hspace*{0.2em}\cellcolor{gray!25}\bf{Prediction task} &
            \hspace*{0.5em}\cellcolor{gray!25}\bf{Images} \\
            \hline\\[-3.8mm]
            Emotion & Rating:$1, 2, 3, 4, 5$  & 4924 $\beta$-maps \\
                    &                         & \textit{collection\_503}\\
            \hline\\[-3.8mm]
            Pain   & Level: $1, 2, 3$  & 84 $\beta$-maps \\
                   &                   & \textit{collection\_504}\\
            \hline\\[-3.8mm]
            Working memory   & face vs place  & 3140 $z$-maps \\
            \hline\\[-3.8mm]
            Gambling   & loss vs reward & 1574 $z$-maps \\
            \hline\\[-3.8mm]
            Relational  & relational vs matching & 1572 $z$-maps \\
            \hline\\[-3.8mm]
            Archi standard  & left vs right hand & 1040 $z$-maps \\
        \end{tabular}
    \end{center}
    \caption{\textbf{Task-fMRI datasets used in predicting stimuli from
        statistical maps analysis.} For each dataset we show the prediction
        task and the number of statistical maps used for prediction.
        \label{tab:task}
    }
\end{table}

\subsection{Image reconstruction}
To be able to train an image reconstruction model we tapped into the largest
and most diverse public database of unthresholded statistical maps -
NeuroVault.org \citep{gorgolewski2015}. After exclusion of non-BOLD,
resting state, meta-analysis,
Human Connectome Project (HCP) \citep{vanessen2013hcp}, UCLA Consortium for
Neuropsychiatric Phenomics\citep{poldrack2016phenome} maps and
semi-automated quality inspection we have curated a
dataset of \textbf{15542} maps.
% 825 of those maps (with no data augmentation) were set aside as a validation set.

\subsection{Task-fMRI}
To predict experimental stimuli from unthresholded brain statistical responses,
we select six diverse task-fMRI studies from which we
predict conditions based on each task. The six studies we select are
summarized on \autoref{tab:task}. For each study, we gather brain responded
images either by downloading them from Neurovault.org \citep{gorgolewski2015}
which are indicated with \textit{collection\_id} on \autoref{tab:task} or by doing
standard analysis \emph{i.e.,} fitting the general linear model (GLM) on task-fMRI
timeseries signals to compute the standardized $z$-maps
\footnote{\url{https://nistats.github.io/}, Nistats package used to fit GLM on
task-fMRI timeseries signals} to various task conditions \citep{friston1995}.

\paragraph{Statistical images from Neurovault} We download collection of
images per subject related to \textbf{Emotion} and \textbf{Pain} experiments
\citep{chang2015emotion}. On each experiment, we focus on predicting the
negative emotional rating (regression) and level of pain (classification) from each
subject. The different levels of emotion and pain are summarized on
\autoref{tab:task}.

\paragraph{Statistical images estimated using GLM} We estimate $z$-maps on
HCP900 \citep{vanessen2012hcpdata} and Individual Brain Charting (IBC)
\citep{pinho2018ibc} projects released task-fMRI datasets. From HCP900, we
estimate \textbf{Working Memory} task-based maps per condition: 0-back faces,
2-back faces, 0-back places, 2-back places. Similarly, on
\textbf{Gambling} \citep{delgado2000gambling} and \textbf{Relational
processing}, we estimate task-based maps per condition: loss, reward,
relational processing and matching respectively. All these maps, we use them
in a 4-class and 2-class classifications task as shown on \autoref{tab:task}.

From IBC, we estimate maps on \textbf{Archi Standard} \citep{pinel2007} motor task
protocol. We use this dataset to probe different prediction setting \emph{i.e.,}
within-subject classification by leaving-one-subject-out. On total of 13
subjects who have undergone multiple sessions, we estimate 80 maps per subject
based on condition to respond via left and right hand button press
to visual and audio instructions. We focus on classifying between left vs right
hand motor maps.

\begin{table}[t]
    \small
    \begin{center}
        \begin{tabular}{c|c|c}
            \hspace*{0.3em}\cellcolor{gray!25}\bf{Rest-fMRI} &
            \hspace*{0.2em}\cellcolor{gray!25}\bf{Prediction task} &
            \hspace*{0.5em}\cellcolor{gray!25}\bf{Images} \\
            \hline\\[-3.8mm]
            HCP900 & High IQ vs Low IQ & 443 subjects \\
            \hline\\[-3.8mm]
            ABIDE  & Autism vs control & 866 subjects \\
            \hline\\[-3.8mm]
            ACPI   & Marijuana use vs control & 126 subjects \\
            \hline\\[-3.8mm]
            ADNI  & Alzheimers vs MCI & 136 subjects \\
            \hline\\[-3.8mm]
            ADNIDOD  & PTSD vs control & 167 subjects \\
            \hline\\[-3.8mm]
            COBRE  & Schizophrenia vs control & 142 subjects \\
            \hline\\[-3.8mm]
            CamCAN  & Age & 626 subjects \\
        \end{tabular}
    \end{center}
    \caption{\textbf{Diverse range of Rest-fMRI datasets used to predict
            targets from functional connectomes.} For each dataset we show the
            classification target and the number of subjects. On CamCAN, we
            predict age from the brain in a regression. IQ - Fluid intelligence,
            PTSD - Post Traumatic Stress Disorder, MCI - Mild Cognitive Impairment.
        \label{tab:rest}
    }
\end{table}

\subsection{Rest-fMRI} We select seven open source rs-fMRI datasets
in order to study predicting diverse targets from functional connectomes. See
\autoref{tab:rest}. The seven targets we study serves to develop imaging-based
biomarkers. We study various outcomes which includes:

\textit{Neuro-degenerative diseases}  -- Alzheimer's Disease Neuroimaging
Initiative\footnote{\url{www.adni-info.org}}
databases \textbf{ADNI} and \textbf{ADNIDOD} \citep{mueller2005}.

\textit{Neuro-psychiatric disorders} -- Autism Brain Imaging Data Exchange database
\textbf{ABIDE} \citep{dimartino2014autism} and Center for Biomedical Research
Excellence\footnote{\url{cobre.mrn.org}} \textbf{COBRE} \citep{calhoun2012}.

\textit{Drug consumption} -- Addiction Connectome Preprocessed
Initiative\footnote{\url{http://fcon_1000.projects.nitrc.org/indi/ACPI/html/}}
\textbf{ACPI}.

\textit{Fluid intelligence} -- Human Connectome Project \textbf{HCP}
\citep{vanessen2013hcp}.

\textit{Brain-aging} -- Cambridge Center for Ageing and Neuroscience
\textbf{CamCAN} \citep{taylor_2017}.

We focus on binary classification problems \emph{i.e.,} predicting a phenotypic
target between two groups on all outcomes except CamCAN where we probe
different setting of predicting age.

\begin{table}[p]
    \small
    \begin{center}
        \begin{tabular}{c|c|c}
            \hspace*{-0.3em}\bf Dataset & \hspace*{0.2em}\bf Prediction target
            & \hspace*{0.5em}\bf Groups \\
            \hline\\[-3.8mm]
            \cellcolor{gray!25} HCP & \cellcolor{gray!25}High IQ vs low IQ & \cellcolor{gray!25}213/230 \\
            \hline\\[-3.8mm]
            ABIDE & Autism vs control & 402/464 \\
            \hline\\[-3.8mm]
            \cellcolor{gray!25}ACPI & \cellcolor{gray!25}Marijuana use vs control & \cellcolor{gray!25}62/64 \\
            \hline\\[-3.8mm]
            ADNI & Alzheimers disease vs MCI & 40/96 \\
            \hline\\[-3.8mm]
            \cellcolor{gray!25}ADNIDOD & \cellcolor{gray!25}PTSD vs control & \cellcolor{gray!25}89/78 \\
            \hline\\[-3.8mm]
            COBRE & Schizophrenia vs control & 65/77 \\
            \cellcolor{gray!25}CamCAN & \cellcolor{gray!25}Age & \cellcolor{gray!25}$24 - 86$ \\
        \end{tabular}
    \end{center}%
    \caption{\textbf{Rest-fMRI datasets and number of subjects per group in
            multiple prediction targets.} PTSD - Post Traumatic Stress
            Disorder, IQ - fluid intelligence, MCI - Mild Cognitive Impairment.
        \label{tab:exp_study_datasets}
    }
\end{table}

\subsection{Encoding}
To do the encoding analysis, we use data from IBC release \citep{pinho2018ibc}
related to visual stimuli based on Rapid-Serial-Visual-Presentation (RSVP)
language task protocol. We use six experimental conditions -- complex
meaningful sentences, simple meaningful sentences, jabberwocky, list of words,
lists of pseudowords, list of non-words -- performed on multi-subjects where
we include 13 subjects in this analysis. The experimental details of RSVP
language protocol are detailed else where \citep{pinho2018ibc}.

\subsection{Meta-analysis}
To use the meta-analysis framework, we collect unthresholded statistical maps of
several cognitive topics from Neurovault.org \citep{gorgolewski2015}. The topics we
collect include -- \textbf{Motor}-task related maps of $1048$,
\textbf{Language}-task related maps of 1031, and \textbf{Face}-areas related
task of $47$ maps --  for each subject respectively after quality inspection.

